Differential Dynamic Programming for Nonlinear Dynamic Games

Dynamic games arise when multiple agents with differing objectives choose control inputs to a dynamic system. Dynamic games model a wide variety of applications in economics, defense, and energy systems. However, compared to single-agent control problems, the computational methods for dynamic games are relatively limited. As in the single-agent case, only very specialized dynamic games can be solved exactly, and so approximation algorithms are required. This paper extends the differential dynamic programming algorithm from single-agent control to the case of non-zero sum full-information dynamic games. The method works by computing quadratic approximations to the dynamic programming equations. The approximation results in static quadratic games which are solved recursively. Convergence is proved by showing that the algorithm iterates sufficiently close to iterates of Newton's method to inherit its convergence properties. A numerical example is provided.

==> di2019differential.aux.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "di2019differential"
%%% End:


==> old.tex <==

\section{Old Stuff}
However, it is common practice for multiplayer games to solve for necessary conditions \cite{frihauf2012nash}\cite{basar1999dynamic}\cite{fershtman1984capital}\cite{gonzalez2016survey}.

The methods considered in this paper are Newton's method for root finding that solves problem \ref{problem:necessary} and DDP for game. Both the methods start from a given trajectory $\bar x$, $\bar u$, where
\begin{align}
  \label{eq:traj}
  \bar x_{k+1} = f_k(\bar x_k, \bar u_{:,k}), \ k = 0, 1, \ldots, T-1
\end{align}
and update the current trajectory input $\bar u$ by $\delta u$. The update step is repeated until convergence for both methods. We denote Newton's method's update by $\delta u^N$ and DDP's update by $\delta u^D$. The letter $N$ is overloaded as it's used to denote both the update for Newton's method and the total time steps. If it appears in the superscript, it means the former and latter if it appears in the subscripts. Note that the solutions given by both methods depend on the initial trajectory. Given different initial trajectories, the methods might converge to different local Nash equilibriums.

\subsection{Shorthand Notations}
We use the following short hand notations throughout this
paper. Subscripts $i$ and $j$ are used as time indices, same as $k$
when we need more two or more time indices. Superscript $l$ is to
denote the $l$th element of a vector, and superscripts such as $1u$,
$1x$, $ux$, $uu$ are used to pick out a corresponding
submatrix/subvector, especially in Jacobians, Hessians and coefficient
matrices for quadratic expressions.



The shorthand notations are
$\delta x_k$ and $\Delta x_k$ are used later as states in an auxiliary dynamic game problem. $A_k$, $B_k$ and $G_k$ capture the first and second order derivatives of the dynamics around $\bar x$ and $\bar u$. $R_k(\delta x_k, \delta u_{:,k})$ is just a shorthand for what appears to be large. $M_{n,k}$ captures the derivatives of cost functions up to second order for each player at every time step. All quantities with subscripts $k$ and $n$ are defined for $k = 0, 1, \ldots, T$ and $n = 1, 2, \ldots, N$

\section{REVIEW OF EXISTING RESULTS}
Here we briefly review two existing results, static quadratic game and the idea of differential dynamic programming for optimal control problem. These ideas are essential building blocks for our proposed DDP method for games. Note that the notations in this section is separate from the rest of this paper unless otherwise noted.
\subsection{Static Quadratic Game}
Static quadratic game \cite{basar1999dynamic} appears in several places throughout this paper. In a static quadratic game, each player has control over its own input $u_n$ and wants to minimize a quadratic cost $J_n(u)$ depending on the collected inputs of all players. $Q_n$ is a positive semi-definite matrices that define the quadratic cost for each player.
\begin{subequations}
  \begin{align}
    J_n(u) =&
              \begin{bmatrix}
                1 \\
                u
              \end{bmatrix}^\top Q_n
    \begin{bmatrix}
      1 \\
      u
    \end{bmatrix} \\
    =&
       \begin{bmatrix}
         1 \\
         u
       \end{bmatrix}^\top
    \begin{bmatrix}
      Q_n^{11} & Q_n^{1u_1} & Q_n^{1u_2} & \cdots & Q_n^{1u_N} \\
      Q_n^{u_11} & Q_n^{u_1 u_1} & Q_n^{u_1 u_2} & \cdots & Q_n^{u_1 u_N} \\
      Q_n^{u_21} & Q_n^{u_2 u_1} & Q_n^{u_2 u _2} & \cdots & Q_n^{u_2 u_N} \\
      \vdots & \vdots & \vdots & \ddots & \vdots \\
      Q_n^{u_N1} & Q_n^{u_N u_1} & Q_n^{u_N u_2} & \cdots & Q_n^{u_N u_N} \\
    \end{bmatrix}
    \begin{bmatrix}
      1 \\
      u
    \end{bmatrix}
  \end{align}
\end{subequations}
The static game also assumes full information structure, which means every player knows the costs for all players. The Nash equilibrium input $u^{\star}$ solves
\begin{align}
  \label{eq:static_q_game_solution}
  \begin{bmatrix}
    Q_1^{u_1 u_1} & Q_1^{u_1 u_2} & \cdots & Q_1^{u_1 u_N} \\
    Q_2^{u_2 u_1} & Q_2^{u_2 u_2} & \cdots & Q_2^{u_2 u_N} \\
    \vdots & \vdots & \ddots & \vdots \\
    Q_N^{u_N u_1} & Q_N^{u_N u_2} & \cdots & Q_N^{u_N u_N} \\
  \end{bmatrix} u^{\star} = H u^{\star} = -
  \begin{bmatrix}
    Q_1^{u1} \\
    Q_2^{u2} \\
    \vdots \\
    Q_N^{uN}
  \end{bmatrix}
\end{align}
The solution exists uniquely if and only if $H$ is invertible.
\subsection{Differential Dynamic Programming (DDP)} \label{sec:DDP}
For a nonlinear dynamic game in general, the exact state-action cost-to-go function $Q_{n, k}(x_k, u_{:,k})$ or state cost-to-go function $V_{n, k}(x_k)$ is hard to solve. Differential dynamical programming \cite{jacobson1968new} was originally proposed to solve optimal control problems, by approximating the state-action cost-to-go function with a quadratic function so the minimization can be done analytically. The same idea applies for game scenarios. The only difference is, instead of solving a minimization problem around the nominal trajectory, we solve for the equilibrium policy, which is also an affine policy as in (\ref{eq:static_q_game_solution}), leaving the resulting state cost-to-go function still quadratic.
\section{Differential Dynamic Programming for Games}
Without further ado, we introduce the DDP method for nonlinear dynamic games. Notice that the method directly works on the dynamic game problem \ref{problem:original}.
\begin{proof}
  We prove lemma \ref{lem:ddp_game_solution} is the solution using DDP idea inductively. For the final time step $k=T$, DDP generates an approximated quadratic state-action cost-to-go function $\tilde Q_{n, T}(x_k, u_{:,k})$ by quadraticizing $c_{n,T}(x_k, u_{:,k})$, which is guaranteed by (\ref{eq:TildeGammaInit}). Assume that (\ref{eq:ddpQ}) holds for $k$, the equilibrium policy gain $\tilde K_k$ and offset $\tilde s_k$ come directly from the result of static quadratic game as in (\ref{eq:static_q_game_solution}), because for this stage, we are equivalently solving a static quadratic game where each player's cost is $\tilde Q_{n,k}(x_k, u_{:,k})$ with its own input $\delta u_{n,k}$.
  The state cost-to-go function $\tilde V_{n,k}(x_k)$ comes by substituting $\delta u_{:,k} = \tilde K_k \delta x_k + \tilde s_k$ into $\tilde Q_{n,k}(x_k, u_{:,k})$, which is purely algebraic.
  \begin{align}
    & \tilde V_{n,k}(x_k) = \tilde Q_{n,k}(x_k, \bar u_{:,k} + \tilde K_k \delta x_k + \tilde s_k) \nonumber \\
    & = \frac{1}{2}
      \begin{bmatrix}
        1 \\
        \delta x \\
        \tilde K_k \delta x_k
      \end{bmatrix}^\top \tilde \Gamma_{n, k}
    \begin{bmatrix}
      1 \\
      \delta x \\
      \tilde K_k \delta x_k + \tilde s_k
    \end{bmatrix} \nonumber \\
    &= \frac{1}{2}
      \begin{bmatrix}
        1 \\
        \delta x \\
        \tilde K_k \delta x_k
      \end{bmatrix}^\top \tilde \Gamma_{n, k}
    \begin{bmatrix}
      1 \\
      \delta x \\
      \tilde K_k \delta x_k
    \end{bmatrix} \nonumber \\
    & \quad +
      \begin{bmatrix}
        0 \\
        0 \\
        \tilde s_k
      \end{bmatrix}^\top \tilde \Gamma_{n, k}
    \begin{bmatrix}
      1 \\
      \delta x \\
      \tilde K_k \delta x_k
    \end{bmatrix} + \frac{1}{2} \tilde s_k^\top \tilde \Gamma_{n,k}^{uu} \tilde s_k \nonumber \\
    &= \frac{1}{2}
      \begin{bmatrix}
        1 \\
        \delta x
      \end{bmatrix}^\top \left(
    \begin{bmatrix}
      1 & 0 & 0 \\
      0 & I & K_k^\top
    \end{bmatrix} \tilde \Gamma_{n, k}
              \begin{bmatrix}
                1 & 0 \\
                0 & I \\
                0 & K_k
              \end{bmatrix} \right)
                    \begin{bmatrix}
                      1 \\
                      \delta x
                    \end{bmatrix} + \nonumber \\
    & \frac{1}{2}
      \begin{bmatrix}
        1 \\
        \delta x
      \end{bmatrix}^\top \left(
    \begin{bmatrix}
      \tilde s_k^\top \tilde \Gamma_{n, k}^{uu} \tilde s_k + 2 \tilde s_k^\top \tilde \Gamma_{n, k}^{u1} & \tilde s_k^\top (\tilde \Gamma_{n, k}^{ux} + \tilde \Gamma_{n, k}^{uu} K_k) \\
      (\tilde \Gamma_{n, k}^{ux} + \tilde \Gamma_{n, k}^{uu} K_k) \tilde s_k & 0
    \end{bmatrix} \right)
                                                                               \begin{bmatrix}
                                                                                 1 \\
                                                                                 \delta x
                                                                               \end{bmatrix} \nonumber \\
    &= \frac{1}{2}
      \begin{bmatrix}
        1 \\
        \delta x_k \\
      \end{bmatrix}^\top \tilde S_{n, k}
    \begin{bmatrix}
      1 \\
      \delta x_k \\
    \end{bmatrix}
  \end{align}
  Thus, (\ref{eq:TildeSDef}) is proven. The stepping back in time of $\tilde \Gamma_{k, n}$ comes from quadraticizing the current stage cost plus the approximated next state cost-to-go function.
  \begin{subequations}
    \label{eq:Q_approx_ddp}
    \begin{align}
      & \tilde Q_{n,k}(x_{k}, u_{k}) = \text{quad}\left( c_{n, k}(x_k, u_{:,k}) + \tilde V_{n,k+1}(f_k(x_k, u_{:,k})) \right)_{\bar x, \bar u} \nonumber \\
      &= \frac{1}{2}
        \begin{bmatrix}
          1 \\
          \delta x_k \\
          \delta u_{:,k}
        \end{bmatrix}^\top M_{n, k}
      \begin{bmatrix}
        1 \\
        \delta x_k \\
        \delta u_{:,k}
      \end{bmatrix} + \text{quad}(\tilde V_{n,k+1}(f_k(x_k, u_{:,k})))_{\bar x, \bar u}
    \end{align}
  \end{subequations}
  By construction, the second order approximation for $f_k(x_k, u_{:,k})$ is
  \begin{align}
    \label{eq:xkp1_approx}
    x_{k+1} = f_k(x_k, u_{:,k}) \approx \bar x_{k+1} + A_k \delta x_k + B_k \delta u_{:,k} + \frac{1}{2} R_k(\delta x_k, \delta u_{:,k})
  \end{align}
  We can substitute (\ref{eq:xkp1_approx}) to $\text{quad}(\tilde V_{n,k+1}(f_k(x_k, u_{:,k})))_{\bar x, \bar u}$ and drop higher order terms to get the quadratic approximation for $\tilde V_{n,k+1}(f_k(x_k, u_{:,k}))$
  \begin{align}
    \label{eq:next_cost_approx_ddp}
    & \ \text{quad}(\tilde V_{n,k+1}(f_k(x_k, u_{:,k})))_{\bar x, \bar u} \nonumber \\
    \approx &
              \begin{bmatrix}
                1 \\
                A_k \delta x_k + B_k \delta u_{:,k} + \frac{1}{2} R_k(\delta x_k, \delta u_{:,k})
              \end{bmatrix}^\top
    \tilde S_{n,k+1} \nonumber \\
    & \quad \quad \quad \quad \quad \quad \quad \quad \quad
      \begin{bmatrix}
        1 \\
        A_k \delta x_k + B_k \delta u_{:,k} + \frac{1}{2} R_k(\delta x_k, \delta u_{:,k})
      \end{bmatrix} \nonumber \\
    \approx &
              \begin{bmatrix}
                1 \\
                A_k \delta x_k + B_k \delta u_{:,k}
              \end{bmatrix}^\top
    \tilde S_{n,k+1}
    \begin{bmatrix}
      1 \\
      A_k \delta x_k + B_k \delta u_{:,k}
    \end{bmatrix} \nonumber \\
    & +
      \begin{bmatrix}
        1 \\
        \mathbf{0}
      \end{bmatrix}^\top \tilde S_{n,k+1}
    \begin{bmatrix}
      0 \\
      R_k(\delta x_k, \delta u_{:,k})
    \end{bmatrix} \nonumber \\
    = &
        \begin{bmatrix}
          1 \\
          \delta x_k \\
          \delta u_{:,k}
        \end{bmatrix}^\top
    \begin{bmatrix}
      \tilde S_{n,k+1}^{11} & \tilde S_{n,k+1}^{1x}A_k & \tilde S_{n,k+1}^{1x}B_k \\
      A_k^\top \tilde S_{n,k+1}^{x1} & A_k^\top \tilde S_{n,k+1}^{xx}A_k & A_k^\top \tilde S_{n,k+1}^{xx} B_k \\
      B_k^\top \tilde S_{n,k+1}^{x1}  & B_k^\top \tilde S_{n,k+1}^{xx}A_k & B_k^\top \tilde S_{n,k+1}^{xx} B_k
    \end{bmatrix}
                                                                            \begin{bmatrix}
                                                                              1 \\
                                                                              \delta x_k \\
                                                                              \delta u_{:,k}
                                                                            \end{bmatrix} \nonumber \\
    & +
      \begin{bmatrix}
        \delta x_k \\
        \delta u_{:,k}
      \end{bmatrix}^\top \tilde D_{n,k}
    \begin{bmatrix}
      \delta x_k \\
      \delta u_{:,k}
    \end{bmatrix} \\
    =& \ \text{quad}(\tilde V_{n,k+1}(f_k(x_k, u_{:,k})))_{\bar x, \bar u}
  \end{align}
  We used the $\approx$ sign because the higher order terms are not exactly balanced as we dropped them along the derivation. Note that $R_k(\delta x_k, \delta u_{:,k})$ is second order in $\delta x_k$ and $\delta u_{:,k}$ so only the cross term of it and constant is kept. Once we substitute (\ref{eq:next_cost_approx_ddp}) back to (\ref{eq:Q_approx_ddp}), it can be easily seen that (\ref{eq:TildeGammaBackprop}) holds true for $k$. Equation (\ref{eq:TildeDDef}) is simply true by construction. All (\ref{eq:ddpMatrices}) have been proven.
\end{proof}

Since the DDP game method approximates the cost-to-go functions and only solves for stage-wise equilibrium instead of overall equilibrium, some questions naturally pop out such as "How good the approximation is?" and "Does state-wise equilibriums form overall equilibrium?". We answer these questions by proving the convergence rate of the proposed method in later sections.

\section{Equivalent Problems and Solutions via Newton's Method}
It is hard to directly work on the convergence rate of the DDP algorithm for games. We know that Newton's method for root finding problems converges quadratically. However, since the solution of Newton's method takes on a very different form from that of DDP, it's still hard to compare them and conclude the convergence rate for DDP. In this section, we show that a direct application of Newton's method to problem \ref{problem:necessary} is equivalent to the solution of a dynamic game problem, which has a similar form to DDP solution of problem \ref{problem:original}.
\subsection{Equivalent Problems}
Problem \ref{problem:necessary} can be solved via Newton's method since it's essentially a root finding problem for the vector function $\mathcal{J}(u)$. Newton's method updates the current $\bar u$ to $\bar u + \delta u^N$ and the update $\delta u^N$ solves the equation

\begin{problem}
  \label{problem:auxiliary_static}
  An auxiliary static game \\
  Each player tries to minimize their own cost
\end{problem}

If we apply the solution to static quadratic game (\ref{eq:static_q_game_solution}), it is obvious that the solution to this game is exactly the Newton's method's update step $\delta u^N$ which solves $\nabla \mathcal{J}(\bar u) \delta u^N = - \mathcal{J}(\bar u)$.

\begin{problem}
  \label{problem:auxiliary_dynamic}
  An auxiliary dynamic game \\
  Each player is trying to minimize its cost
\end{problem}

This auxiliary dynamic game problem is the key to our proof, as its solution is equivalent to the Newton's method's update and the form is close to that of DDP solution so that they can be compared.

\begin{lemma}
  Problem \ref{problem:auxiliary_static} and problem \ref{problem:auxiliary_dynamic} are equivalent.
\end{lemma}

\begin{proof}
  \end{proof}

\begin{lemma}
  \label{lem:auxiliary_dynamic_solution0}
  $\delta u^N$ such that $\nabla \mathcal{J}(\bar u) \delta u^N = - \mathcal{J}(\bar u)$ is the solution to problem \ref{problem:auxiliary_dynamic}.
\end{lemma}
\begin{proof}
  Since the update via Newton's method $\delta u^N$ to $\nabla \mathcal{J}(\bar u) \delta u^N = - \mathcal{J}(\bar u)$ for problem \ref{problem:necessary}
  is the solution to problem \ref{problem:auxiliary_static}, and the two auxiliary problems are equivalent, $\delta u^N$ is also the solution to problem \ref{problem:auxiliary_dynamic}.
\end{proof}

\subsection{Dynamic Programming Solution to the Auxiliary Dynamic Game}
We give the direct solution to problem \ref{problem:auxiliary_dynamic} via dynamic programming, prove it and compare it with the solution via DDP in section \ref{sec:DDP}. According to lemma \ref{lem:auxiliary_dynamic_solution0}, this solution is equivalent to the Newton update step $\delta u^N$.

\begin{lemma}
  \label{lem:newton_dp_solution}
  The solution to problem \ref{problem:auxiliary_dynamic} via dynamic programming has the following form

  \begin{subequations}
    \label{eq:newton_dp_solution}
    State-action cost-to-go functions
    Equilibrium affine policy
    \begin{align}
      \label{eq:newton_dp_minimizer}
      \delta u_{:,k} = K_k \delta x_k + s_k
    \end{align}
  \end{subequations}
  where the matrices are found
  and $n = 1, 2, \ldots, N$ and $k = 0, 1, \ldots, T$.
\end{lemma}

\begin{proof}
  The proof is very similar to the proof for DDP solution. Solving $V_{n,k}(\delta x_k, \Delta x_k)$ based on $Q_{n,k}(\delta x_k, \Delta x_k, \delta u_{:,k})$ is the same as in the DDP solution proof, since the extra terms of $\Delta x_k$ are not coupled with $\delta u_{:,k}$ and everything else has the exact same form. We omit the proof for it.
  The stepping back in time of $Q_k(\delta x_k, \Delta x_k, \delta u_{:,k})$ is slightly different because of the extra terms related to $\Delta x_k$.
  \begin{subequations}
    \label{eq:newton_dp_backprop}
    \begin{align}
      & Q_{n,k}(\delta x_k, \Delta x_k, \delta u_{:,k}) \\
      &= \frac{1}{2} \left(
        \begin{bmatrix}
          1 \\
          \delta x_k \\
          \delta u_{:,k}
        \end{bmatrix}^T
      M_{n,k}
      \begin{bmatrix}
        1 \\
        \delta x_k \\
        \delta u_{:,k}
      \end{bmatrix} + M^{1k}_{n,k} \Delta x_k \right) \nonumber \\
      & \quad + V_{n, k+1}(\delta x_{k+1}, \Delta x_{k+1}) \\
      &= \frac{1}{2} \left(
        \begin{bmatrix}
          1 \\
          \delta x_k \\
          \delta u_{:,k}
        \end{bmatrix}^T
      M_{n,k}
      \begin{bmatrix}
        1 \\
        \delta x_k \\
        \delta u_{:,k}
      \end{bmatrix} + M^{1k}_{n,k} \Delta x_k \right) \nonumber \\
      & \quad + V_{n,k+1}(A_k \delta{x}_k + B_k  \delta{u}_k, A_k \Delta x_{k}  + R_k(\delta x_k, \delta u_{:,k})) \\
      &= \frac{1}{2} \left(
        \begin{bmatrix}
          1 \\
          \delta x_k \\
          \delta u_{:,k}
        \end{bmatrix}^T
      M_{n,k}
      \begin{bmatrix}
        1 \\
        \delta x_k \\
        \delta u_{:,k}
      \end{bmatrix} + M^{1k}_{n,k} \Delta x_k \right) \nonumber \\
      & \quad + \frac{1}{2} \left(
        \begin{bmatrix}
          1 \\
          A_k \delta{x}_k + B_k \delta{u}_k
        \end{bmatrix}^T S_{n,k+1}
      \begin{bmatrix}
        1 \\
        A_k \delta{x}_k + B_k \delta{u}_k
      \end{bmatrix}\right) \nonumber \\
      & \quad + \frac{1}{2} \left( \Omega_{n,k+1} A_k \Delta x_{k}  + \Omega_{n,k+1} R_k(\delta x_k, \delta u_{:,k})) \right) \\
      &= \frac{1}{2} \left(
        \begin{bmatrix}
          1 \\
          \delta x_k \\
          \delta u_{:,k}
        \end{bmatrix}^T
      M_{n,k}
      \begin{bmatrix}
        1 \\
        \delta x_k \\
        \delta u_{:,k}
      \end{bmatrix} \right) + \nonumber \\
      & \frac{1}{2}
        \begin{bmatrix}
          1 \\
          \delta{x}_k \\
          \delta u_{:,k}
        \end{bmatrix}^T
      \begin{bmatrix}
        S^{11}_{n,k+1} & S^{1x}_{n,k+1} A_k & S^{1x}_{n,k+1} B_k \\
        A^\top_k S^{x1}_{n,k+1} & A^\top_k S^{xx}_{n,k+1} A_k & A^\top_k S^{xx}_{n,k+1} B_k \\
        B^\top_k S^{x1}_{n,k+1} & B^\top_k S^{xx}_{n,k+1} A_k & B^\top_k S^{xx}_{n,k+1} B_k
      \end{bmatrix}
                                                                \begin{bmatrix}
                                                                  1 \\
                                                                  \delta{x}_k \\
                                                                  \delta u_{:,k}
                                                                \end{bmatrix} \nonumber \\
      & \quad + \frac{1}{2} \left( (M^{1k}_{n,k} + \Omega_{n,k+1} A_k) \Delta x_{k} \right) \nonumber \\
      & \quad + \frac{1}{2} \left( \sum_{l=0}^n \Omega_{n,k+1}^l
        \begin{bmatrix}
          \delta x_k \\
          \delta u_{:,k}
        \end{bmatrix}^T
      G_k^l
      \begin{bmatrix}
        \delta x_k \\
        \delta u_{:,k}
      \end{bmatrix} \right) \\
      &= \frac{1}{2} \left(
        \begin{bmatrix}
          1 \\
          \delta x_k \\
          \delta u_{:,k}
        \end{bmatrix}^T
      M_{n,k}
      \begin{bmatrix}
        1 \\
        \delta x_k \\
        \delta u_{:,k}
      \end{bmatrix} \right) + \nonumber \\
      & \frac{1}{2}
        \begin{bmatrix}
          1 \\
          \delta{x}_k \\
          \delta u_{:,k}
        \end{bmatrix}^T
      \begin{bmatrix}
        S^{11}_{n,k+1} & S^{1x}_{n,k+1} A_k & S^{1x}_{n,k+1} B_k \\
        A^\top_k S^{x1}_{n,k+1} & A^\top_k S^{xx}_{n,k+1} A_k & A^\top_k S^{xx}_{n,k+1} B_k \\
        B^\top_k S^{x1}_{n,k+1} & B^\top_k S^{xx}_{n,k+1} A_k & B^\top_k S^{xx}_{n,k+1} B_k
      \end{bmatrix}
                                                                \begin{bmatrix}
                                                                  1 \\
                                                                  \delta{x}_k \\
                                                                  \delta u_{:,k}
                                                                \end{bmatrix} \nonumber \\
      & \quad + \frac{1}{2} \left( (M^{1k}_{n,k} + \Omega_{n,k+1} A_k) \Delta x_{k} \right) \nonumber \\
      & \quad + \frac{1}{2} \left(
        \begin{bmatrix}
          \delta x_k \\
          \delta u_{:,k}
        \end{bmatrix}^T
      D_{n,k}
      \begin{bmatrix}
        \delta x_k \\
        \delta u_{:,k}
      \end{bmatrix} \right)
    \end{align}
  \end{subequations}
  So (\ref{eq:GammaDef})(\ref{eq:newton_dp_solution_omega1})(\ref{eq:newton_dp_solution_D}) are true.
\end{proof}

Notice that the equilibrium strategy given by (\ref{eq:newton_dp_minimizer}) is the same as the update step from a direct Newton's method root finding algorithm (\ref{eq:direct_newton}) since we have proven the equivalency of the two problems they respectively solve.

Problem \ref{problem:auxiliary_dynamic} has a quadratic cost function. Even though the dynamics of $\Delta x$ contains a quadratic form of the input $\delta u$ and $\delta x$, but because $\Delta x$ only appears linearly in the cost function, the cost-to-go functions are still quadratic and hence can be solved. Notice that unlike the DDP solution to problem \ref{problem:original}, which is approximate because we are quadraticizing the state-action cost-to-go function at each step, the solution (\ref{eq:newton_dp_solution}) to problem \ref{problem:auxiliary_dynamic} is exact because the problem is already quadraticized around the given trajectory.

\section{CONVERGENCE OF DIFFERENTIAL DYNAMIC PROGRAMMING FOR GAMES}
DDP is known to converge quadratically to locally optimal solution \cite{liao1991convergence} just like Newton's method \cite{murray1984differential}. We prove that DDP for games shares the same convergence rate in this section. We know that Newton's method for root finding enjoys a quadratic convergence rate \cite{nocedal2006numerical}. For a given set of inputs $\bar u$ that's close to the equilibrium $u^{\star}$, i.e.  Newton's method finds the next input $\delta u^N$ and DDP finds $\delta u^D$. The step by step solution $\delta u^N_k$ in (\ref{eq:newton_dp_minimizer}) serves as a bridge between Newton's method solution and DDP, since it's equivalent to Newton's method solution and has the same form as the DDP solution $\delta u^D_k$. We prove that $\delta u^D_k = \delta u^N_k + O(\epsilon^2)$, concluding that DDP update has the same quadratic convergence rate as Newton's root finding. In this section, we use superscripts $^N$ or $^D$ to denote the source of $\delta x_k$ and $\delta u_k$. Superscript $^D$ indicates variables from solution of DDP method in (\ref{eq:ddp_solution}) and $^N$ indicates those from (\ref{eq:newton_dp_solution}).

\subsection{Closeness of Newton's Method to DDP} \label{sec:closeness}
We first derive a few useful results which we'll use later in this chapter.

First, we bound the spectral radius of $F_k^{-1}$ from above
\begin{align}
  \rho(F_k^{-1}) \leq \hat F
\end{align}
where $\hat F$ is a constant. Consider inverting $\nabla_{u} \mathcal{J}(u)$ in Newton's method by successively eliminating $\delta u_{:,k}$ for $k=T,T-1,\ldots,0$. The
$F_k$ matrices are exactly the matrices which would be inverted when eliminating $\delta u_{:,k}$. Since $\nabla_u \mathcal{J}(u)$ is Lipschitz continuous, its eigenvalues are bounded away from zero in a neighborhood of $u^{\star}$. It follows that the eigenvalues of $F_K$ must also be bounded away from zero and $F_k^{-1}$ is bounded above.

Secondly, we assert that
\begin{align}
  \label{eq:omega_equiv}
  \Omega_{n,k} = \frac{\partial}{\partial x_k}\Big|_{\bar x, \bar u} \sum_{i=k}^{T} c_{n,i}(x_i, u_{:,i})
\end{align}
which means $\Omega_{n,k}$ captures the first-order effect of $x_k$ on the sum of all later costs for each player. $\Omega_{n,k}$ is constructed according to (\ref{eq:newton_dp_solution_omega0})(\ref{eq:newton_dp_solution_omega1}). Equation (\ref{eq:omega_equiv}) is true for $k = T$ by construction. We proof by induction and assume that (\ref{eq:omega_equiv}) holds for $k+1$, i.e. $\Omega_{n,k+1} = \frac{\partial}{\partial x_{k+1}}\Big|_{\bar x, \bar u} \sum_{i={k+1}}^{T} c_{n,i}(x_i, u_{:,i})$, then
\begin{subequations}
  \begin{align}
    & \Omega_{n,k} = M_{n,k} + \Omega_{n, k+1} A_k \\
    & = \frac{\partial c_{n,k}(x_k, u_{:,k})}{x_k}\Big|_{\bar x, \bar u} + \left( \frac{\partial}{\partial x_{k+1}} \sum_{i=k+1}^{T} c_{n,i}(x_i, u_{:,i}) \right) \frac{\partial x_{k+1}}{\partial x_{k}} \Big|_{\bar x, \bar u} \\
    & = \frac{\partial c_{n,k}(x_k, u_{:,k})}{x_k}\Big|_{\bar x, \bar u} + \left( \frac{\partial}{\partial x_{k}}\Big|_{\bar x, \bar u} \sum_{i=k+1}^{T} c_{n,i}(x_i, u_{:,i}) \right) \\
    & = \frac{\partial}{\partial x_k}\Big|_{\bar x, \bar u} \sum_{i=k}^{T} c_{n,i}(x_i, u_{:,i})
  \end{align}
\end{subequations}
Therefore, (\ref{eq:omega_equiv}) holds for $k$. And by induction, all $k = 0,1, \ldots, T$.

The third useful result is that
\begin{align}
  \label{eq:J_grad_small}
  M^{1u}_{n,k} + \Omega_{n,k+1} B_k = \frac{\partial J_n(u)}{\partial u_{:,k}}\Big|_{\bar u} = O(\epsilon)
\end{align}
$\frac{\partial J_n(u)}{\partial u_{:,k}}\Big|_{\bar u} = O(\epsilon)$ is true because $J_n(u)$ is twice differentiable hence Lipschitz, i.e.
\begin{align}
  \Big|\Big| \frac{J_n(u)}{\partial u_{:,k}}\Big|_{\bar u} - \frac{J_n(u)}{\partial u_{:,k}}\Big|_{u^{\star}} \Big|\Big|^2 \leq \text{constant} \cdot \|\bar u - u^{\star}\|^2 = O(\epsilon)
\end{align}
The first equality holds because
\begin{subequations}
  \begin{align}
    \frac{\partial J(u)}{\partial u_{:,k}}\Big|_{\bar u} =& \frac{\partial }{\partial u_{:,k}}\Big|_{\bar x, \bar u} \sum_{i=0}^T c_{n,i}(x_i, u_{:,i}) = \frac{\partial }{\partial u_{:,k}}\Big|_{\bar x, \bar u} \sum_{i=k}^T c_{n,i}(x_i, u_{:,i}) \\
    =& \frac{\partial }{\partial u_{:,k}}\Big|_{\bar x, \bar u} c_{n,k}(x_k, u_{:,k}) + \frac{\partial }{\partial u_{:,k}}\Big|_{\bar x, \bar u} \sum_{i=k+1}^T c_{n,i}(x_i, u_{:,i}) \\
    =& M_{n,k}^{1u} + \frac{\partial }{\partial x_{k+1}} \Big|_{\bar x, \bar u} \sum_{i=k+1}^T c_{n,i}(x_i, u_{:,i}) \frac{\partial x_{k+1}}{\partial u_{:,k}} \Big|_{\bar x, \bar u} \\
    =& M^{1u}_{n,k} + \Omega_{n,k+1} B_k
  \end{align}
\end{subequations}
Now we are equipped to bound $\delta u_k^N$ and $\delta u_k^D$.

\begin{lemma}
  \label{lem:closeness_backward}
  Assume $\bar u$ is in the neighborhood of the true solution $u^{\star}$, such that  $\epsilon = \norm{\bar u - u^{\star}}$ is small, then
  \begin{subequations}
    \label{eq:closeness}
    \begin{align}
      \label{eq:close_D}
      \tilde D_{n,k} &= D_{n,k} + O(\epsilon) \\
      \label{eq:close_S0}
      S^{1x}_{n,k} &= \Omega_{n,k} + O(\epsilon) \\
      \label{eq:close_S1}
      \tilde S^{1x}_{n,k} &= \Omega_{n,k} + O(\epsilon) \\
      \label{eq:close_S2}
      \tilde S^{1x}_{n,k} &= S^{1x}_{n,k} + O(\epsilon^2) \\
      \label{eq:close_S3}
      \tilde S_{n,k} &= S_{n,k} + O(\epsilon) \\
      \label{eq:close_gamma0}
      \begin{bmatrix}
        \tilde \Gamma^{1x}_{n,k} & \tilde \Gamma^{1u}_{n,k}
      \end{bmatrix} &=
                      \begin{bmatrix}
                        \Gamma^{1x}_{n,k} & \Gamma^{1u}_{n,k}
                      \end{bmatrix} + O(\epsilon^2) \\
      \label{eq:close_gamma1}
      \tilde \Gamma_{n,k} &= \Gamma_{n,k} + O(\epsilon)\\
      \label{eq:close_gamma2}
      \Gamma_{n,k}^{1u} &= O(\epsilon) \\
      \label{eq:close_gamma3}
      \tilde \Gamma_{n,k}^{1u} &= O(\epsilon) \\
      \label{eq:close_F}
      \tilde F_k &= F_k + O(\epsilon) \\
      \label{eq:close_P}
      \tilde P_k &= P_k + O(\epsilon) \\
      \label{eq:close_H0}
      \tilde H_k &= H_k + O(\epsilon^2) \\
      \label{eq:close_H1}
      \tilde H_k &= O(\epsilon) \\
      \label{eq:close_H2}
      H_k &= O(\epsilon) \\
      \label{eq:close_s0}
      \tilde s_k &= s_k + O(\epsilon^2) \\
      \label{eq:close_s1}
      \tilde s_k &= O(\epsilon) \\
      \label{eq:close_s2}
      s_k &= O(\epsilon) \\
      \label{eq:close_K}
      \tilde K_k &= K_k + O(\epsilon)
    \end{align}
  \end{subequations}
\end{lemma}

\begin{proof}
  \label{proof:closeness}
  We prove the closeness by induction. \\

  For $k = T$, because of the way these variables are constructed, they are identical, i.e.
  \begin{subequations}
    \begin{align}
      \Gamma_{n,T} =& \tilde \Gamma_{n,T} \\
      F_T =& \tilde F_T \\
      P_T =& \tilde P_T \\
      H_T =& \tilde H_T \\
      s_T =& \tilde s_T \\
      K_T =& \tilde K_T \\
      S_{n,T} =& \tilde S_{n,T}
    \end{align}
  \end{subequations}
  So we have  (\ref{eq:close_S2})(\ref{eq:close_S3})(\ref{eq:close_gamma0})(\ref{eq:close_gamma1})(\ref{eq:close_F})(\ref{eq:close_P})(\ref{eq:close_H0})(\ref{eq:close_s0})(\ref{eq:close_K}) hold for $k = T$.

  We also know that
  \begin{align}
    M_{n,T}^{1u} = \frac{\partial c_{n,T}}{\partial u_T} = \frac{\partial J_n(u)}{\partial u_T}=O(\epsilon)
  \end{align} where the first equality is by construction, the second is true because $u_T$ only appears in $J_n(u)$ in $c_{n,T}$. By construction, $\Gamma_{n,T}^{1u} = \tilde \Gamma_{n,T}^{1u} = M_{n,T}^{1u} = O(\epsilon)$, so (\ref{eq:close_gamma2})(\ref{eq:close_gamma3}) are true for $k = T$. \\
  Similarly, $H_T$ and $\tilde H_T$ are constructed from $\Gamma_{n,T}^{u1}$ and $\tilde \Gamma_{n,T}^{u1}$, so (\ref{eq:close_H1})(\ref{eq:close_H2}) are true for $k=T$.

  Because $F_k^{-1}$ is bounded above, $s_T = - F_T^{-1} H_T = - F_T^{-1} O(\epsilon) = O(\epsilon)$. Similarly, $\tilde s_T = O(\epsilon)$. Equations (\ref{eq:close_s1})(\ref{eq:close_s2}) are true for $k=T$.

  From (\ref{eq:newton_dp_solution_S}) and $\Gamma_{n,T} = M_{n,T}$, we can get
  \begin{subequations}
    \begin{align}
      S_{n,T}^{1x} =& M_{n,T}^{1x} + M_{n,T}^{1u} K_T + s_T^\top ( M_{n,T}^{ux} + M_{n,T}^{uu} K_T ) \\
      =& \Omega_{n,T} + O(\epsilon) K_T + O(\epsilon) ( M_{n,T}^{ux} + M_{n,T}^{uu} K_T ) \\
      =& \Omega_{n,T} + O(\epsilon)
    \end{align}
  \end{subequations}
  because $M_{n,T}$ is bounded. Hence (\ref{eq:close_S0}) is true. Further, (\ref{eq:close_S1}) is also true.

  The time indices for $D_{n,T-1}$ and $\tilde D_{n,T-1}$ go to a maximum of $T-1$, so to prove things inductively, we need (\ref{eq:close_D}) to hold for $k=T-1$.The difference between constructions of $D_{n,T-1}$ and $\tilde D_{n,T-1}$ is in that the former uses $\Omega_{n,T}$ and the later uses $\tilde S_{n,T}^{1x}$. But since we've proven $\Omega_{n,T} = \tilde S_{n,T}^{1x} + O(\epsilon)$, and $G_{T-1}$ is bounded, we can also conclude $D_{n,T-1} = \tilde D_{n,T-1} + O(\epsilon)$. Therefore (\ref{eq:close_D}) is true for $k = T-1$.

  So far, we've proved that for the last step, either $k = T$ or $k= T -1$, (\ref{eq:closeness}) is true. Assuming except for (\ref{eq:close_D}), (\ref{eq:closeness}) is true for $k+1$ and (\ref{eq:close_D}) is true for $k$. If we can prove all equations hold one step back, our proof by induction would be done.

  Assume (\ref{eq:close_D}) holds for $k$ and other equations in (\ref{eq:closeness}) hold for $k+1$. Readers be aware that we'll use these assumptions implicitly in the derivations following.

  From (\ref{eq:GammaDef}) we can get
  \begin{subequations}
    \begin{align}
      \Gamma_{n,k}^{1u} =& M_{k,T}^{1u} + S_{n,k+1}^{1x} B_k \\
      =& M_{k,T}^{1u} + \Omega_{n,k+1} B_k + O(\epsilon) B_k \\
      =& O(\epsilon)
    \end{align}
  \end{subequations}
  Here we used (\ref{eq:J_grad_small}). Similarly, we can prove $\tilde \Gamma_{n,k}^{1u} = O(\epsilon)$. So (\ref{eq:close_gamma2})(\ref{eq:close_gamma3}) hold for $k$.

  From (\ref{eq:GammaDef})(\ref{eq:TildeGammaBackprop}) we can compute the difference between $\tilde \Gamma_{n,k}$ and $\Gamma_{n,k}$ as
  \begin{subequations}
    \begin{align}
      & \ \tilde \Gamma_{n,k} - \Gamma_{n,k} \nonumber \\
      = &
          \begin{bmatrix}
            \tilde S_{n, k+1}^{11} - S_{n, k+1}^{11} & \mathbf{0} & \mathbf{0} \\
            A_k^\top (\tilde S_{n,k+1}^{x1} - S_{n,k+1}^{x1}) & \mathbf{0} & \mathbf{0} \\
            B_k^\top  (\tilde S_{n,k+1}^{x1} - S_{n,k+1}^{x1}) & \mathbf{0} & \mathbf{0}
          \end{bmatrix} \nonumber \\
      & +
        \begin{bmatrix}
          \mathbf{0} & (\tilde S_{n,k+1}^{1x} - S_{n,k+1}^{1x})A_k & \mathbf{0} \\
          \mathbf{0} & A_k^\top (\tilde S_{n,k+1}^{xx} - S_{n,k+1}^{xx})A_k + (\tilde D_k^{xx} - D_k^{xx}) & \mathbf{0} \\
          \mathbf{0} & B_k^\top (\tilde S_{n,k+1}^{xx} - S_{n,k+1}^{xx}) A_k + (\tilde D_k^{ux} - D_k^{ux}) & \mathbf{0}
        \end{bmatrix} \nonumber \\
      & +
        \begin{bmatrix}
          \mathbf{0} & \mathbf{0} & (\tilde S_{n,k+1}^{1x} - S_{n,k+1}^{1x})B_k \\
          \mathbf{0} & \mathbf{0} & A_k^\top (\tilde S_{n,k+1}^{xx} - S_{n,k+1}^{xx}) B_k + (\tilde D_k^{xu} - D_k^{xu}) \\
          \mathbf{0} & \mathbf{0} & B_k^\top (\tilde S_{n,k+1}^{xx} - S_{n,k+1}^{xx}) B_k + (\tilde D_k^{uu} - D_k^{uu})
        \end{bmatrix} \\
      =& \begin{bmatrix}
        O(\epsilon) & A_k O(\epsilon^2) & B_k O(\epsilon^2) \\
        A_k^\top O(\epsilon^2) & A_k^\top O(\epsilon) A_k  + O(\epsilon) & A_k^\top O(\epsilon) B_k  + O(\epsilon) \\
        B_k^\top O(\epsilon^2)  & B_k^\top O(\epsilon) A_k + O(\epsilon) & B_k^\top O(\epsilon) B_k + O(\epsilon)
      \end{bmatrix} \\
      =&
         \begin{bmatrix}
           O(\epsilon) & O(\epsilon^2) & O(\epsilon^2) \\
           O(\epsilon^2) & O(\epsilon) & O(\epsilon) \\
           O(\epsilon^2) & O(\epsilon) & O(\epsilon)
         \end{bmatrix}
    \end{align}
  \end{subequations}
  from which we can see that (\ref{eq:close_gamma0})(\ref{eq:close_gamma1}) are true.
  Once we proved the closeness between $\tilde \Gamma_{n,k}$ and $\Gamma_{n,k}$ and the specific terms are $O(\epsilon)$, i.e. (\ref{eq:close_gamma0}) to (\ref{eq:close_gamma3}), because of they way they are constructed from $\tilde \Gamma_{n,k}$ and $\Gamma_{n,k}$, we are safe to say
  \begin{subequations}
    \begin{align}
      \tilde F_k &= F_k + O(\epsilon) \\
      \tilde P_k &= P_k + O(\epsilon) \\
      \tilde H_k &= H_k + O(\epsilon^2) \\
      \tilde H_k &= O(\epsilon) \\
      H_k &= O(\epsilon)
    \end{align}
  \end{subequations}
  Therefore, (\ref{eq:close_F})(\ref{eq:close_P})(\ref{eq:close_H0})(\ref{eq:close_H1})(\ref{eq:close_H2}) are true for $k$.

  Now that we have the results with $F_k$, $\tilde F_k$, $H_k$, $\tilde H_k$, $P_k$ and $\tilde P_k$, we can move to what are immediately following, i.e. $s_k$, $\tilde s_k$, $K_k$ and $\tilde K_k$.
  \begin{align}
    s_k =& - F_k^{-1} H_k = - F_k^{-1} O(\epsilon) = O(\epsilon)
  \end{align}
  which is true because $F_k^{-1}$ is bounded above. Similarly, we have $\tilde s_k = O(\epsilon)$. Equations (\ref{eq:close_s1})(\ref{eq:close_s2}) are true.

  \begin{subequations}
    \begin{align}
      \tilde s_k &= - \tilde F_k^{-1} \tilde H_k = - (F_k + O(\epsilon))^{-1} (H_k + O(\epsilon^2)) \\
                 &= - (F_k^{-1} + O(\epsilon)) (H_k + O(\epsilon^2)) \\
                 &= - F_k^{-1} H_k + F_k^{-1} O(\epsilon^2) + H_k O(\epsilon) + O(\epsilon^2) \\
                 &= s_k + O(\epsilon^2) \\
      \tilde K_k &= - \tilde F_k^{-1} \tilde P_k = - (F_k + O(\epsilon))^{-1} (P_k + O(\epsilon)) \\
                 &= - (F_k^{-1} + O(\epsilon)) (P_k + O(\epsilon)) \\
                 &= - F_k^{-1} P_k + (F_k^{-1} + P_k) O(\epsilon) + O(\epsilon^2) \\
                 &= K_k + O(\epsilon)
    \end{align}
  \end{subequations}
  Equation (\ref{eq:close_s0})(\ref{eq:close_K}) are true for $k$.

  Now we are equipped to get closeness/small results for $S_{n,k}$ and $\tilde S_{n,k}$.
  \begin{subequations}
    \begin{align}
      & \ \tilde S_{n,k} - S_{n,k} \nonumber \\
      =&
         \begin{bmatrix}
           1 & 0 & 0 \\
           0 & I & \tilde K_k^\top
         \end{bmatrix} \tilde \Gamma_{n, k}
                   \begin{bmatrix}
                     1 & 0 \\
                     0 & I \\
                     0 & \tilde K_k
                   \end{bmatrix} -
                         \begin{bmatrix}
                           1 & 0 & 0 \\
                           0 & I & K_k^\top
                         \end{bmatrix} \Gamma_{n, k}
                                   \begin{bmatrix}
                                     1 & 0 \\
                                     0 & I \\
                                     0 & K_k
                                   \end{bmatrix} \nonumber \\
      & +
        \begin{bmatrix}
          \tilde s_k^\top \tilde \Gamma_{n, k}^{uu} \tilde s_k + 2 \tilde s_k^\top \tilde \Gamma_{n, k}^{u1} - s_k^\top \Gamma_{n, k}^{uu} s_k - 2 s_k^\top \Gamma_{n, k}^{u1} & \mathbf{0} \\
          (\tilde \Gamma_{n, k}^{xu} + \tilde \Gamma_{n, k}^{uu} \tilde K_k) \tilde s_k - (\Gamma_{n, k}^{ux} + \Gamma_{n, k}^{uu} K_k)^\top s_k & \mathbf{0}
        \end{bmatrix} \nonumber \\
      & +
        \begin{bmatrix}
          \mathbf{0} & \tilde s_k^\top (\tilde \Gamma_{n, k}^{ux} + \tilde \Gamma_{n, k}^{uu} \tilde K_k) - s_k^\top (\Gamma_{n, k}^{ux} + \Gamma_{n, k}^{uu} K_k) \\
          \mathbf{0} & \mathbf{0}
        \end{bmatrix} \\
      =&
         \begin{bmatrix}
           \tilde \Gamma_{n,k}^{11} & \tilde \Gamma_{n,k}^{1x} + \tilde \Gamma_{n,k}^{1u} \tilde K \\
           \tilde \Gamma_{n,k}^{x1} + \tilde K^\top \tilde \Gamma_{n,k}^{u1} & \tilde \Gamma_{n,k}^{xx} + 2 \tilde \Gamma_{n,k}^{xu} \tilde K + \tilde K^\top \tilde \Gamma_{n,k}^{uu} \tilde K
         \end{bmatrix} \nonumber \\
      & -
        \begin{bmatrix}
          \Gamma_{n,k}^{11} & \Gamma_{n,k}^{1x} + \Gamma_{n,k}^{1u} K \\
          \Gamma_{n,k}^{x1} + K^\top \Gamma_{n,k}^{u1} & \Gamma_{n,k}^{xx} + 2 \Gamma_{n,k}^{xu} K + K^\top \Gamma_{n,k}^{uu} K
        \end{bmatrix} \nonumber \\
      & +
        \begin{bmatrix}
          O(\epsilon) & O(\epsilon^2) \\
          O(\epsilon) & 0
        \end{bmatrix} \\
      =&
         \begin{bmatrix}
           O(\epsilon) & O(\epsilon^2) \\
           O(\epsilon^2) & O(\epsilon)
         \end{bmatrix} \\
    \end{align}
  \end{subequations}
  So that (\ref{eq:close_S2})(\ref{eq:close_S3}) are true for $k$.

  \begin{subequations}
    \begin{align}
      & S_{n,k}^{1x} = M_{n,k}^{1x} + S_{n,k+1}^{1x} A_k + \Gamma_{n,k}^{1u} K_k + s_k^\top ( \Gamma_{n,k}^{ux} + \Gamma_{n,k}^{uu} K_k ) \\
      & = M_{n,k}^{1x} + \Omega_{n,k+1} A_k + A_k O(\epsilon) \nonumber \\
      & \quad + K_k O(\epsilon) +  (\Gamma_{n,k}^{ux} + \Gamma_{n,k}^{uu} K_k) O(\epsilon) \\
      & = \Omega_{n,k} + O(\epsilon)
    \end{align}
  \end{subequations}
  Therefore, (\ref{eq:close_S0}) holds and then naturally (\ref{eq:close_S1}) holds.

  We continue to prove that $\tilde D_{n,k-1}$ and $D_{n, k-1}$ are close, which is true because
  \begin{subequations}
    \begin{align}
      \tilde D_{n,k-1} =& \sum_{l=1}^{n_x} \tilde S_{n,k}^{1x^l} G_k^l \\
      =& \sum_{l=1}^{n_x} (\Omega_{n,k}^l + O(\epsilon)) G_k^l \\
      =& \sum_{l=1}^{n_x} \Omega_{n,k}^l G_k^l + O(\epsilon) \\
      =& D_{n,k-1} + O(\epsilon)
    \end{align}
  \end{subequations}
  So (\ref{eq:close_D}) is true.
\end{proof}

Next we introduce the final lemma we need to say that DDP has quadratic convergence rate.

\begin{lemma}
  \label{lem:input_closeness_forward}
  Let $\delta u^N$ and $\delta u^D$ be the updates by Newton's method and DDP method and $\bar u - u^{\star} = \epsilon$, then
  \begin{subequations}
    \label{eq:closeness_forward}
    \begin{align}
      \label{eq:DDP_approx_states}
      \delta x_{k+1}^D =& A_k \delta x_k^D + B_k \delta u_k^D + O(\epsilon^2) \\
      \label{eq:newton_approx_states}
      \delta x_{k+1}^N =& A_k \delta x_k^N + B_k \delta u_k^N + O(\epsilon^2) \\
      \label{eq:input_small_newton}
      \delta u_k^N = O(\epsilon) \\
      \label{eq:input_small_ddp}
      \delta u_k^D = O(\epsilon) \\
      \label{eq:state_small_newton}
      \delta x_k^N = O(\epsilon) \\
      \label{eq:state_small_ddp}
      \delta x_k^D = O(\epsilon) \\
      \label{eq:input_step_close}
      \delta u_k^N - \delta u_k^D =& O(\epsilon^2)\\
      \label{eq:state_step_close}
      \delta x_k^N - \delta x_k^D =& O(\epsilon^2)\\
      \label{eq:close_update_newton_DDP}
      \delta u^N - \delta u^D =& O(\epsilon^2) \\
      \label{eq:classic_newton_convergence}
      \|\bar u + \delta u^N - u^{\star}\| =& O(\epsilon^2). \\
      \label{eq:DDP_convergence}
      \|\bar u + \delta u^D - u^{\star}\| =& O(\epsilon^2).
    \end{align}
  \end{subequations}
  From the above bounding equations, we can conclude that DDP method update converges quadratically.
\end{lemma}
\begin{proof}
  Equation (\ref{eq:DDP_approx_states}) comes directly from the Taylor series expansion of (\ref{eq:DDP_state}) and (\ref{eq:newton_approx_states}) from (\ref{eq:newton_dp_dynamics0}).

  We prove (\ref{eq:input_small_newton}) to (\ref{eq:state_step_close}) by induction. For $k=0$, $\delta x_{0}^N = \delta x_{0}^D = 0$ and $\delta u_{0}^N = s_0,\  \delta x_{0}^D = \tilde s_0$. We know from lemma \ref{lem:closeness_backward} that $s_0 = \tilde s_0 + O(\epsilon^2)$, $s_0 = O(\epsilon)$ and $\tilde s_0 = O(\epsilon)$,  so (\ref{eq:input_small_newton}) to (\ref{eq:state_step_close}) hold for $k=0$. Assume (\ref{eq:input_small_newton}) to (\ref{eq:state_step_close}) hold for $k$, then
  \begin{subequations}
    \begin{align}
      \delta u^N_{k+1} &= K_{k+1} \delta x^N_k + s_{k+1} = O(\epsilon) \\
      \delta u^D_{k+1} &= \tilde K_{k+1} \delta x^N_k + \tilde s_{k+1} = O(\epsilon) \\
      \delta x^N_{k+1} =& A_k \delta x^N_k + B_k \delta u^N_k + O(\epsilon^2) = O(\epsilon) \\
      \delta x^D_{k+1} =& A_k \delta x^D_k + B_k \delta u^D_k + O(\epsilon^2) = O(\epsilon) \\
      \delta u^N_{k+1} - \delta u^D_{k+1} =& K_k \delta x^N_{k} - \tilde K_k \delta x^D_{k} + s_k - \tilde s_k \\
      =& K_k \delta x^N_k - (K_k + O(\epsilon)) (\delta x^N_k + O(\epsilon^2)) \nonumber \\
                       & + O(\epsilon^2) \\
      =& O(\epsilon) \delta x^N_k + O(\epsilon^2) \\
      =& O(\epsilon^2) \\
      \delta x^N_{k+1} - \delta x^D_{k+1} =& A_k ( \delta x^N_{k} - \delta x^D_{k} ) + B_k ( \delta u^N_{k} - \delta u^D_{k} ) + O(\epsilon^2) \nonumber \\
      =& O(\epsilon^2)
    \end{align}
  \end{subequations}\\
  So (\ref{eq:input_small_newton}) to (\ref{eq:state_step_close}) hold for $k+1$ and the proof by induction is done. Equation (\ref{eq:close_update_newton_DDP}) comes directly as a result. Equation (\ref{eq:classic_newton_convergence}) is classic convergence analysis for Newton's method \cite{nocedal2006numerical}. Equation (\ref{eq:DDP_convergence}) follows directly from (\ref{eq:close_update_newton_DDP})(\ref{eq:classic_newton_convergence}).
\end{proof}

Since we've proven that Newton's method and DDP method update are quadratically close and that Newton's method converges quadratically to the solution of problem \ref{problem:necessary}, we conclude that DDP method also converges to the solution of problem \ref{problem:necessary} quadratically.




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "di2019differential.tex"
%%% End:

